Shaped Four-Dimensional Modulation Formats for Optical Fiber Communication Systems

We review the design of multidimensional modulations by maximizing generalized mutual information and compare the maximum transmission reach of recently introduced 4D formats. A model-based optimization for nonlinear-tolerant 4D modulations is also discussed.

==> table.tex <==
\def\arraystretch{1}
\begin{table}[!htbp]
\caption{Simulation parameters.}
\begin{center}
\label{tab:syspar}
%\scalebox{0.9}{
{\footnotesize
\begin{tabular}{lr}
%\hline

%\multicolumn{2}{|c|}{\emph{Transmitter Parameters}}& %\multicolumn{2}{|c|}{\emph{Fiber Channel Parameters}}  \\ 
%\hline \hline
%{\bf Parameter Name} & {\bf Value} & {\bf Parameter Name} & {\bf Value}  \\
%\hline 
%Wavelength-division multiplexing Channels & 11 & Attenuation  & 0.2 dB/km  \\
%\hline
%Symbol Rate & 41.79 Gbaud  & Dispersion Parameter  & 17 ps/nm/km\\
%\hline
%Root-raised-cosine Roll-Off factor & 0.1& Nonlinearity Parameter  & 1.3 1/(W$\cdot$km)\\
%\hline
%Channel Frequency Spacing & 50 GHz & Fiber Span Length & 80 km  \\
%\hline
%Center Wavelength  & 1550nm & EDFA Noise Figure & 5 dB\\
%\hline
%Wavelength band & 1539.4-1560.8nm (81 channels) \\

% \hline
% \hline
%\multicolumn{2}{|c|}{{Simulation Parameters}}\\
%\hline 
%\hline 
\toprule
{\bf Parameter name} & {\bf Value}  \\
% \hline
\midrule
WDM Channels & 11    \\
% \hline
Symbol rate & {45~GBd}   \\
% \hline
Root-raised-cosine roll-off factor & {1}{\%} \\
% \hline
Channel frequency spacing & {50~GHz}      \\
% \hline
Center wavelength  & {1550~nm}  \\
%Aggregate launch power & {9.5}{dBm}\\
% \hline
% \\
%\hline
Attenuation & {0.21~dB/km} \\
% \hline
Dispersion parameter & {16.9~ps nm$^{-1}$km $^{-1}$} \\
% \hline
Nonlinearity parameter & {1.31~W $^{-1}$ km $^{-1}$} \\
% \hline
Fibre span length & 80~km \\
% \hline
EDFA noise figure & {5~dB} \\
% \hline\hline
\toprule
%\multicolumn{2}{|c|}{\emph{Numerical Parameters}}  \\
%\hline
%SSF Spatial Step Size & 100 m \\
%\hline
%Simulation Bandwidth & 512 GHz \\
%\hline
\end{tabular}
}
%}
\end{center}
\end{table}
